Multimodal Prompt Optimization: Why Not Leverage Multiple Modalities for MLLMs

Large Language Models (LLMs) have shown remarkable success, and their multimodal expansions (MLLMs) further unlock capabilities spanning images, videos, and other modalities beyond text. However, despite this shift, prompt optimization approaches, designed to reduce the burden of manual prompt crafting while maximizing performance, remain confined to text, ultimately limiting the full potential of MLLMs. Motivated by this gap, we introduce the new problem of multimodal prompt optimization, which expands the prior definition of prompt optimization to the multimodal space defined by the pairs of textual and non-textual prompts. To tackle this problem, we then propose the Multimodal Prompt Optimizer (MPO), a unified framework that not only performs the joint optimization of multimodal prompts through alignment-preserving updates but also guides the selection process of candidate prompts by leveraging earlier evaluations as priors in a Bayesian-based selection strategy. Through extensive experiments across diverse modalities that go beyond text, such as images, videos, and even molecules, we demonstrate that MPO outperforms leading text-only optimization methods, establishing multimodal prompt optimization as a crucial step to realizing the potential of MLLMs.

==> Tables/response_example2.tex <==
% \begin{table*}[t]
%   \centering
%   \scriptsize
%   \renewcommand{\arraystretch}{1.0} 
%   \begin{tabularx}{\linewidth}{@{}X@{}}
%     \toprule
%     \multicolumn{1}{c}{\textbf{Task Example: CUB(Auklet) Classification}} \\
    
% \midrule

%     \textbf{Image Query} \\
%       \adjustbox{valign=t}{%
%         \includegraphics[width=0.2\linewidth]{Figures/qualitative/image_ex_auklet.jpg}%
%       }
%       \hfill 
%       \begin{minipage}[t]{0.75\linewidth}
%         \textbf{Ground Truth}: \textcolor{blue}{\textbf{Crested Auklet}} \newline
%         \vspace{0.2cm} 
%         \textbf{Key Features}:
%         \begin{itemize}[nosep, leftmargin=*]
%             \item Dark plumage
%             \item Curved crest of feathers
%             \item Orange beak
%         \end{itemize}
%       \end{minipage}
%       \\
%       \midrule
%     \textbf{Optimized Prompt (MPO) (Score: 80.3)} \\
%     \begin{minipage}[t]{0.28\linewidth}
%         \vspace{0pt}
%         \includegraphics[width=\linewidth]{Figures/qualitative/auklet.jpg}
%         % \vspace{0.1cm} \centering \footnotesize{\textit{Hybrid Reference}}
%     \end{minipage}%
%     \hfill
%     \begin{minipage}[t]{0.68\linewidth}
%     \tiny
%         Analyze the provided hybrid image of auklet species and classify the bird in the target image into one of the following categories: [`parakeet auklet', `rhinoceros auklet', `crested auklet', `least auklet']. Focus on the following critical visual features:
        
%         \vspace{0.5em}
%         1. \textbf{Bill Shape}: Prioritize the size and shape of the bill, comparing it directly with the examples in the hybrid image. Be specific about curvature and thickness.
        
%         \vspace{0.5em}
%         2. \textbf{Plumage Color}: Observe the overall body color and any variations, noting how these compare to the reference images.
        
%         \vspace{0.5em}
%         3. \textbf{Body Patterns}: Identify unique markings or patterns on the body, ensuring to highlight any significant differences that may aid in classification.
        
%         \vspace{0.5em}
%         Use the hybrid image as a guide for your comparison and classification. Clearly mention any distinguishing traits that support your decision, and ensure to prioritize bill shape in cases of ambiguity.
%     \end{minipage} \\
%     \cdashline{1-1}[0.5pt/1pt]\rule{-2pt}{3.0ex}
%     \textbf{Response}\\
%     \tiny
%         The bird in the target image can be classified as a ``crested auklet'' based on the following observations: \\
%         \addlinespace[3pt]
%         1. \textbf{Bill Shape}: The bill is relatively short and thick, with a slight curve at the tip. \textcolor{figgreen}{\textbf{This matches the description of the ``crested auklet'' in the reference image, which has a similar bill shape but with a more pronounced curve}}. The ``rhinoceros auklet'' also has a thick bill but with a more pronounced curve, while the ``parakeet auklet'' and ``least auklet'' have thinner bills.\\
%         \addlinespace[3pt]
%         2. \textbf{Plumage Color}: The overall body color is dark, almost black, with some lighter areas around the neck and underparts. \textcolor{figgreen}{\textbf{This is consistent with the ``crested auklet'' in the reference image.}} The ``rhinoceros auklet'' has a similar dark plumage, but the ``parakeet auklet'' and ``least auklet'' have lighter plumage.\\
%         \addlinespace[3pt]
%         3. \textbf{Body Patterns}: The most distinctive feature of the ``crested auklet'' is the presence of a crest on its head, which is clearly visible in the target image. The ``parakeet auklet'' and ``least auklet'' do not have crests, and the ``rhinoceros auklet'' has a shorter crest compared to the ``crested auklet''.\\
%         \addlinespace[3pt]
%         In conclusion, the combination of the short and thick bill, dark plumage, and the presence of a crest on the head strongly supports the classification of the bird in the target image as a \textcolor{figgreen}{\textbf{``crested auklet''}}.
%     \\
% \midrule
%         % --- BASELINE (SEE) SECTION ---
%         \textbf{Optimized Prompt (SEE)} \textit{(Score: 50.0)}  \\
%         \tiny
%         Classify the content of the target image based on the provided choices of bird species: [`parakeet auklet', `rhinoceros auklet', `crested auklet', `least auklet'].
        
%         \vspace{0.5em}
%         \textbf{Comprehensive Guidelines for Classification:}
%         \vspace{0.5em}
        
%         \textbf{1. Physical Characteristics}: 
%         \vspace{0.3em}
        
%         \textbf{- Parakeet Auklet}: Look for a small bird (approx. 23 cm), with a striking blue bill and a notable yellow eyebrow stripe. Its compact body and vibrant colors are key identifiers. 
        
        
%         \textbf{- Rhinoceros Auklet}: This medium-sized bird (about 35 cm) has a stout body and a distinctive horn-like projection on its bill during breeding season. It typically weighs around 700 grams, so note its robust build.
        
        
%         \textbf{- Crested Auklet}: Identify this species by its long, curved crest of feathers and dark plumage, roughly 30 cm in size. Weighing about 300 grams, it is often found in colonies, so observe any social behaviors. 
        
        
%         \textbf{- Least Auklet}: The smallest of the auklets (around 20 cm), it features short wings and a stubby bill, weighing about 130 grams. Its petite size and subtle coloration are distinguishing traits.
        
%         \vspace{0.3em}
%         \textbf{2. Habitat and Behavior}: Focus on typical habitats such as coastal regions and rocky cliffs. Note behaviors like diving and feeding. For instance, the \textbf{Rhinoceros Auklet} may exhibit aggressive diving, while the \textbf{Crested Auklet} shows unique social interactions.
        
%         \vspace{0.3em}
%         \textbf{3. Visual Cues}: Pay attention to specific visual markers such as bill shape, color, and the feather crest on the \textbf{Crested Auklet}. Consistently assess the color of the feet and overall body size.
        
%         \vspace{0.3em}
%         \textbf{4. Common Confusions}: Be aware that the \textbf{Rhinoceros Auklet} appears more robust than the slender \textbf{Least Auklet}. Additionally, plumage colors may vary under different lighting conditions.
        
%         \vspace{0.3em}
%         \textbf{5. Cross-Verification Process}: Use a methodical approach to verify classification. For instance, check if dark plumage corresponds with the bill shape and size of the suspected species, and look for unique features.
        
%         \vspace{0.3em}
%         \textbf{6. Key Features to Focus On}: Highlight aspects such as beak shape, feather patterns, and eye color during evaluation.
        
%         \vspace{0.3em}
%         \textbf{7. Narrow Down Options}: If the image shows features that could apply to multiple species, focus on the most probable candidates based on observed visual cues and behaviors.
        
%         \vspace{0.3em}
%         \textbf{8. Confidence Level}: Indicate your confidence in the classification as ``certain,'' ``likely,'' ``uncertain,'' or ``doubtful.'' Justify your confidence by detailing which specific features influenced your assessment.
        
%         \vspace{0.3em}
%         \textbf{9. Step-by-Step Checklist for Classification}: Use this systematic checklist: Observe the size and body structure; Note the bill's color and shape; Examine plumage patterns and unique features (e.g., crests); Consider the observed habitat and behaviors; Cross-reference traits with the characteristics of all species.
        
%         \vspace{0.3em}
%         \textbf{10. Hypothetical Example Scenarios}: Provide examples of images and a breakdown of classifications according to the guidelines, illustrating effective application of features and observations.
        
%         \vspace{0.3em}
%         Please provide the identified species name and your confidence level in the classification. \\

%     \cdashline{1-1}[0.5pt/1pt]\rule{-2pt}{3.0ex}
%         \textbf{Response} \\
%         \tiny
%         Based on the provided image, let's analyze the bird step-by-step using the comprehensive guidelines:
        
%         \vspace{0.4em}
%         \textbf{1. Physical Characteristics}: The bird has a robust body, which aligns with the Rhinoceros Auklet being described as medium-sized (about 35 cm) and having a stout body. The bill is orange with a black tip, which is characteristic of the Rhinoceros Auklet. There is a noticeable horn-like projection on the bill, which is a key feature of the Rhinoceros Auklet during the breeding season.
        
%         \vspace{0.3em}
%         \textbf{2. Habitat and Behavior}: The bird is perched on a rocky cliff, which is consistent with the Rhinoceros Auklet's habitat preference. The posture and behavior do not provide additional specific clues but do not contradict the identification either.
        
%         \vspace{0.3em}
%         \textbf{3. Visual Cues}: The bill shape and color match the description of the Rhinoceros Auklet. The overall body structure and size are consistent with the Rhinoceros Auklet.
        
%         \vspace{0.3em}
%         \textbf{4. Common Confusions}: The Least Auklet is much smaller and has a shorter bill, which does not match the image. The Crested Auklet has a long, curved crest, which is not present here. The Parakeet Auklet is smaller and has a distinct yellow eyebrow stripe, which is not seen here.
        
%         \vspace{0.3em}
%         \textbf{5. Cross-Verification Process}: The combination of the robust body, orange bill with a black tip, and the horn-like projection strongly supports the identification of the Rhinoceros Auklet.
        
%         \vspace{0.3em}
%         \textbf{6. Key Features to Focus On}: The bill shape and color are critical features for this identification.
        
%         \vspace{0.3em}
%         \textbf{7. Narrow Down Options}: The image clearly matches the Rhinoceros Auklet based on the physical characteristics and visual cues.
        
%         \vspace{0.3em}
%         \textbf{8. Confidence Level}: Given the clear match with the Rhinoceros Auklet's physical characteristics and the absence of any conflicting features, I am confident in the classification.
        
%         \vspace{0.5em}
%         \textbf{Conclusion:}
        
%         The identified species is the \textcolor{red}{\textbf{Rhinoceros Auklet}}, and my confidence level in this classification is \textbf{certain}.
%     \\
%     \bottomrule
%   \end{tabularx}
%   \caption{Visualization of the SEE result on the CUB(Auklet) dataset.}
%   \label{tab:response_example_auklet_see}
% \end{table*}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table*}[t]
%   \centering
%   \scriptsize
%   \renewcommand{\arraystretch}{1.0} 
%   \begin{tabularx}{\linewidth}{@{} p{0.1\linewidth} X @{}}
%     \toprule
%     \multicolumn{2}{c}{\textbf{Task Example: CUB(Auklet) Classification}} \\
%     \midrule
%      % --- OURS (MPO) SECTION ---
%     \textbf{Optimized Prompt (MPO)} 
    
%     \textit{(Score: 80.3)} 
%     & 

%     \begin{minipage}[t]{0.28\linewidth}
%         \vspace{0pt}
%         \includegraphics[width=\linewidth]{Figures/qualitative/auklet.jpg}
%         % \vspace{0.1cm} \centering \footnotesize{\textit{Hybrid Reference}}
%     \end{minipage}%
%     \hfill
%     \begin{minipage}[t]{0.68\linewidth}
%         Analyze the provided hybrid image of auklet species and classify the bird in the target image into one of the following categories: [`parakeet auklet', `rhinoceros auklet', `crested auklet', `least auklet']. Focus on the following critical visual features:
        
%         \vspace{0.5em}
%         1. \textbf{Bill Shape}: Prioritize the size and shape of the bill, comparing it directly with the examples in the hybrid image. Be specific about curvature and thickness.
        
%         \vspace{0.5em}
%         2. \textbf{Plumage Color}: Observe the overall body color and any variations, noting how these compare to the reference images.
        
%         \vspace{0.5em}
%         3. \textbf{Body Patterns}: Identify unique markings or patterns on the body, ensuring to highlight any significant differences that may aid in classification.
        
%         \vspace{0.5em}
%         Use the hybrid image as a guide for your comparison and classification. Clearly mention any distinguishing traits that support your decision, and ensure to prioritize bill shape in cases of ambiguity.
        
%     \end{minipage} \\
    
% \midrule
%     \textbf{Image Query} & 
%       \adjustbox{valign=t}{%
%         \includegraphics[width=0.2\linewidth]{Figures/qualitative/image_ex_auklet.jpg}%
%       }
%       \hfill 
%       \begin{minipage}[t]{0.75\linewidth}
%         \textbf{Ground Truth}: \textcolor{blue}{\textbf{Crested Auklet}} \newline
%         \vspace{0.2cm} 
%         \textbf{Key Features}:
%         \begin{itemize}[nosep, leftmargin=*]
%             \item Dark plumage
%             \item Curved crest of feathers
%             \item Orange beak
%         \end{itemize}
%       \end{minipage}
%       \\
% \midrule
%         \textbf{Response}
%     & 
%         The bird in the target image can be classified as a ``crested auklet'' based on the following observations: \\
%         \addlinespace[3pt]
%         & 1. \textbf{Bill Shape}: The bill is relatively short and thick, with a slight curve at the tip. \textcolor{figgreen}{\textbf{This matches the description of the ``crested auklet'' in the reference image, which has a similar bill shape but with a more pronounced curve}}. The ``rhinoceros auklet'' also has a thick bill but with a more pronounced curve, while the ``parakeet auklet'' and ``least auklet'' have thinner bills.\\
%         \addlinespace[3pt]
%         & 2. \textbf{Plumage Color}: The overall body color is dark, almost black, with some lighter areas around the neck and underparts. \textcolor{figgreen}{\textbf{This is consistent with the ``crested auklet'' in the reference image.}} The ``rhinoceros auklet'' has a similar dark plumage, but the ``parakeet auklet'' and ``least auklet'' have lighter plumage.\\
%         \addlinespace[3pt]
%         & 3. \textbf{Body Patterns}: The most distinctive feature of the ``crested auklet'' is the presence of a crest on its head, which is clearly visible in the target image. The ``parakeet auklet'' and ``least auklet'' do not have crests, and the ``rhinoceros auklet'' has a shorter crest compared to the ``crested auklet''.\\
%         \addlinespace[3pt]
%         &  In conclusion, the combination of the short and thick bill, dark plumage, and the presence of a crest on the head strongly supports the classification of the bird in the target image as a \textcolor{figgreen}{\textbf{``crested auklet''}}.
%     \\
%     \bottomrule
%   \end{tabularx}
%   \caption{Visualization of the MPO result on the CUB(Auklet) dataset.}
%   \label{tab:response_example_auklet_mpo}
% \end{table*}



% \begin{table*}[t]
%   \centering
%   \scriptsize
%   \renewcommand{\arraystretch}{1.0} 
%   \begin{tabularx}{\linewidth}{@{} p{0.1\linewidth} X @{}}
%     \toprule
%     \multicolumn{2}{c}{\textbf{Task Example: CUB(Grosbeak) Classification}} \\
    
% \midrule

%         % --- BASELINE (SEE) SECTION ---
%         \textbf{Optimized Prompt (SEE)} 
        
%         \textit{(Score: 96.7)} 
%     &   
%         Identify the species of the bird in the given image using the options provided. Please respond with the bird's name exactly as it is listed (e.g., `rose breasted grosbeak'). 

%         \vspace{0.5em}
%         Make sure to write the name precisely as it appears in the choices, without any extra punctuation or modifications. Pay attention to distinctive features such as color patterns, markings, and size to accurately identify the bird.
        
%         \vspace{0.5em}        
%         If you find that the bird in the image does not match any of the listed options, please state `not identifiable' rather than guessing. Ensure that your answer is selected only from the choices provided and refrain from inferring details about the species.
        
%         \vspace{0.5em}        
%         After determining the bird, verify that your response is among the listed options before you submit it.
%         \\

% \midrule

%     \textbf{Image Query} & 
%       \adjustbox{valign=t}{%
%         \includegraphics[width=0.2\linewidth]{Figures/qualitative/image_ex_grosbeak.jpg}%
%       }
%       \hfill 
%       \begin{minipage}[t]{0.75\linewidth}
%         \textbf{Ground Truth}: \textcolor{blue}{\textbf{Evening Grosbeak}} \newline
%         \vspace{0.2cm} 
%         \textbf{Key Features}:
%         \begin{itemize}[nosep, leftmargin=*]
%             \item White wing patches
%             \item Yellow body color
%         \end{itemize}
%       \end{minipage}
%       \\
      
% \midrule

%         \textbf{Response}
%     & 
%         \textcolor{red}{\textbf{rose breasted grosbeak}}
        
%     \\
%     \bottomrule
%   \end{tabularx}
%   \caption{Visualization of the SEE result on the CUB(Grosbeak) dataset.}
%   \label{tab:response_example_grosbeck_see}
% \end{table*}




% \begin{table*}[t]
%   \centering
%   \scriptsize
%   \renewcommand{\arraystretch}{1.0} 
%   \begin{tabularx}{\linewidth}{@{} p{0.1\linewidth} X @{}}
%     \toprule
%     \multicolumn{2}{c}{\textbf{Task Example: CUB (Grosbeak) Classification}} \\
%     \midrule
%     \textbf{Image Query} & 
%       \adjustbox{valign=t}{%
%         \includegraphics[width=0.2\linewidth]{Figures/qualitative/image_ex_grosbeak.jpg}%
%       }
%       \hfill 
%       \begin{minipage}[t]{0.75\linewidth}
%         \textbf{Ground Truth}: \textcolor{blue}{\textbf{Evening Grosbeak}} \newline
%         \vspace{0.2cm} 
%         \textbf{Key Features}:
%         \begin{itemize}[nosep, leftmargin=*]
%             \item White wing patches
%             \item Yellow body color
%         \end{itemize}
%       \end{minipage}
%       \\
%     \midrule
%      % --- OURS (MPO) SECTION ---
%     \textbf{Optimized Prompt (MPO)} 
    
%     \textit{(Score: 100.0)} 
%     & 

%     \begin{minipage}[t]{0.2\linewidth}
%         \vspace{0pt}
%         \includegraphics[width=\linewidth]{Figures/qualitative/grosbeak.jpg}
%         % \vspace{0.1cm} \centering \footnotesize{\textit{Hybrid Reference}}
%     \end{minipage}%
%     \hfill
%     \begin{minipage}[t]{0.78\linewidth}
%     Classify the bird in the target image by comparing it with the hybrid reference image of grosbeaks. Follow these refined steps for accurate classification.
    
%     \vspace{0.5em} 
%     1. \textbf{Identify the Grosbeak Group}: Refer to the hybrid image that displays the Rose Breasted Grosbeak, Pine Grosbeak, Blue Grosbeak, and Evening Grosbeak. Familiarize yourself with the specific traits of each species, including color patterns and markings.
    
%     \vspace{0.5em} 
%     2. \textbf{Analyze Visual Features}: Focus on these critical features of the target bird: 
    
%     \vspace{0.2em} 
%     \quad -- \textbf{Dominant Color and Markings}: Note the primary color and any distinctive patterns, such as throat colors or wing designs. 
    
%     \vspace{0.2em} 
%     \quad -- \textbf{Beak Characteristics}: Compare the shape and size of the beak with those in the reference image, as these can vary significantly among species. 
    
%     \vspace{0.2em} 
%     \quad -- \textbf{Body Size Comparison}: Assess the body size of the target bird relative to the reference birds, ensuring accurate size comparisons. 
    
%     \vspace{0.5em} 
%     3. \textbf{Feature Prioritization}: 
    
%     \vspace{0.2em} 
%     \quad -- Prioritize color patterns first, as they are often the most telling feature. 
    
%     \vspace{0.2em} 
%     \quad -- If colors are similar, evaluate beak shape and size next. 
    
%     \vspace{0.2em} 
%     \quad -- Finally, consider body size. If the target bird does not closely match any reference species, provide the name of the closest match or indicate `unknown', based on the following criteria: 
    
%     \vspace{0.2em} 
%     \quad  \quad -- Closeness is determined by the degree of similarity across all analyzed features, with color being the primary factor, followed by beak shape and size. 
    
%     \vspace{0.5em} 
%     After analyzing these features, provide the name of the bird species that most closely matches the visual characteristics observed in the target image, supported by specific observations from the hybrid reference image.\\
%     \end{minipage} \\
%     \cdashline{1-2}[0.5pt/1pt]\rule{-2pt}{3.0ex}
%         \textbf{Response}
%     & 
%         The bird in the target image has a predominantly yellow body with black wings and a white patch on its chest. Its beak is short and conical, suitable for seed-eating. \textcolor{blue}{\textbf{Comparing these features with the hybrid reference image of grosbeaks}}, the bird most closely resembles the \textbf{Evening Grosbeak}. The yellow coloration, black wings, and white chest patch are characteristic of this species. Therefore, the bird in the target image is classified as an \textcolor{blue}{\textbf{Evening Grosbeak}}. \\
%     \midrule
%         % --- BASELINE (SEE) SECTION ---
%         \textbf{Optimized Prompt (SEE)} 
        
%         \textit{(Score: 96.7)} 
%     &   
%         Identify the species of the bird in the given image using the options provided. Please respond with the bird's name exactly as it is listed (e.g., `rose breasted grosbeak'). 

%         \vspace{0.5em}
%         Make sure to write the name precisely as it appears in the choices, without any extra punctuation or modifications. Pay attention to distinctive features such as color patterns, markings, and size to accurately identify the bird.
        
%         \vspace{0.5em}        
%         If you find that the bird in the image does not match any of the listed options, please state `not identifiable' rather than guessing. Ensure that your answer is selected only from the choices provided and refrain from inferring details about the species.
        
%         \vspace{0.5em}        
%         After determining the bird, verify that your response is among the listed options before you submit it.
%         \\
%     \cdashline{1-2}[0.5pt/1pt]\rule{-2pt}{3.0ex}
%     \textbf{Response}  & \textcolor{red}{\textbf{rose breasted grosbeak}} \\
%     \bottomrule
%   \end{tabularx}
%   \caption{Visualization of the MPO result on the CUB(Grosbeak) dataset.}
%   \label{tab:response_example_grosbeck_mpo}
% \end{table*}
